CliMB: An AI-enabled Partner for Clinical Predictive Modeling

Despite its significant promise and continuous technical advances, real-world applications of artificial intelligence (AI) remain limited. We attribute this to the "domain expert-AI-conundrum": while domain experts, such as clinician scientists, should be able to build predictive models such as risk scores, they face substantial barriers in accessing state-of-the-art (SOTA) tools. While automated machine learning (AutoML) has been proposed as a partner in clinical predictive modeling, many additional requirements need to be fulfilled to make machine learning accessible for clinician scientists. To address this gap, we introduce CliMB, a no-code AI-enabled partner designed to empower clinician scientists to create predictive models using natural language. CliMB guides clinician scientists through the entire medical data science pipeline, thus empowering them to create predictive models from real-world data in just one conversation. CliMB also creates structured reports and interpretable visuals. In evaluations involving clinician scientists and systematic comparisons against a baseline GPT-4, CliMB consistently demonstrated superior performance in key areas such as planning, error prevention, code execution, and model performance. Moreover, in blinded assessments involving 45 clinicians from diverse specialties and career stages, more than 80% preferred CliMB over GPT-4. Overall, by providing a no-code interface with clear guidance and access to SOTA methods in the fields of data-centric AI, AutoML, and interpretable ML, CliMB empowers clinician scientists to build robust predictive models. The proof-of-concept version of CliMB is available as open-source software on GitHub: https://github.com/vanderschaarlab/climb.

==> Log/scratch.tex <==

\subsubsection*{Example 1: Data exploration}

\noindent This example demonstrates \textit{CliMB}'s approach to getting a detailed and relevant data analysis via feedback from the user and the available tools (EDA and descriptive statistics).

\mygap

\noindent \textbf{Summary of work up to this point:} The user's file has been loaded, and the alignment of the system's capabilities and the user's intended research question has been confirmed.

\mydots

\begin{assistantbox}
\assistant \texttt{Planning step}
\end{assistantbox}

\begin{assistantbox}
\assistant Let's start by listing all the columns in the dataset. I'll generate code that loads the dataset and prints out the names of all the columns, one by one. This will help you see which columns are available for analysis. \\

\generatedCode
\begin{lstlisting}
import pandas as pd

# Load the dataset
data = pd.read_csv("kidney_train.csv")

# Print the names of all the columns, one by one
print("List of all columns in the dataset:")
for column in data.columns:
    print(column)
\end{lstlisting}
\end{assistantbox}

\begin{execbox}
\codeExecOut
\codeExecSuccess
\begin{lstlisting}[style=codeoutput]
List of all columns in the dataset:
DONOR_ID
DAGE
DSEX

... shortened for brevity ...

Recip_Second_DQ_Broad
Recip_Second_DQ_Split
recip_first_Bw
\end{lstlisting}
\end{execbox}
% DETHNIC
% HYPERTENSION
% DGRP
% DRET_CREAT
% DCOD
% DBMI
% RECIP_ID
% RAGE
% RSEX
% RETHNIC
% RBMI
% PRD
% WAIT_TIME
% GRAFT_NO
% TX_ID
% TX_YR
% HLA_MM
% CIT_MINS
% CRF_TX
% organ_type
% A_0
% ALI_0
% C_0
% M_0
% O_0
% OKI_0
% P_0
% T_0
% A_3
% C_3
% M_3
% O_3
% P_3
% S_3
% T_3
% eGFR3
% eGFR12
% REJECTION
% DGF
% GSURV
% GCENS
% COF
% RCOD
% TX_TYPE
% organs_dntd
% ORGANS_TXD
% PAST_DIABETES
% PAST_HYPERTENSION
% Donor_First_A_Broad
% Donor_First_A_Split
% Donor_Second_A_Broad
% Donor_Second_A_Split
% Donor_First_B_Broad
% Donor_First_B_Split
% Donor_Second_B_Broad
% Donor_Second_B_Split
% Donor_First_C_Broad
% Donor_First_C_Split
% Donor_First_DR_Broad
% Donor_First_DR_Split
% Donor_Second_DR_Broad\texttt{$<$letter$>$\_$<$number$>$}
% Donor_Second_DR_Split
% Donor_First_DQ_Broad
% Donor_First_DQ_Split
% Donor_Second_DQ_Broad
% Donor_Second_DQ_Split
% Donor_first_Bw
% Donor_Second_Bw
% Recip_First_A_Broad
% Recip_First_A_Split
% Recip_Second_A_Broad
% Recip_Second_A_Split
% Recip_First_B_Broad
% Recip_First_B_Split
% Recip_First_C_Broad
% Recip_First_C_Split
% Recip_First_DR_Broad
% Recip_First_DR_Split
% Recip_Second_DR_Broad
% Recip_Second_DR_Split
% Recip_First_DQ_Broad
% Recip_First_DQ_Split

\begin{assistantbox}
\assistant Now that you've seen the list of columns in the dataset, would you like to exclude certain columns from the analysis, or conversely, only keep certain columns? If so, please specify which columns you'd like to exclude or keep.
\end{assistantbox}

\noindent The system provides an opportunity for the user to review the features in the dataset early in the pipeline, and to select a subset of these as needed.

\begin{userbox}
\user I want to remove columns that have a name like $<$letter$>$\_$<$number$>$. I also want to remove columns that start with Recip\_ or Donor\_.
\end{userbox}

\begin{assistantbox}
\assistant Understood. I will generate code to remove columns that have names like \texttt{$<$letter$>$\_$<$number$>$} and those that start with \texttt{Recip\_} or \texttt{Donor\_}. The modified dataset will be saved with a suffix \texttt{\_user\_cols} in the filename. \\

\generatedCode
\begin{lstlisting}
import pandas as pd
import re

# Load the dataset
data = pd.read_csv("kidney_train.csv")

# Columns to exclude based on the specified patterns
exclude_patterns = [r'^[A-Z]_\d+$', r'^Recip_', r'^Donor_']

# Compile regex patterns
compiled_patterns = [re.compile(pattern) for pattern in exclude_patterns]

# Determine which columns to drop
columns_to_drop = [column for column in data.columns if any(pattern.match(column) for pattern in compiled_patterns)]

# Drop the specified columns
data_modified = data.drop(columns=columns_to_drop)

# Save the modified dataset
data_modified.to_csv("kidney_train_user_cols.csv", index=False)

print(f"Columns removed: {len(columns_to_drop)}")
print("Modified dataset saved as 'kidney_train_user_cols.csv'.")
\end{lstlisting}
\end{assistantbox}

\begin{execbox}
\codeExecOut
\codeExecSuccess
\begin{lstlisting}[style=codeoutput]
Columns removed: 49
Modified dataset saved as 'kidney_train_user_cols.csv'.
\end{lstlisting}
\end{execbox}

\begin{toolbox}
\toolExecOut{EDA} \\

\toolLogs
\begin{lstlisting}[style=codeoutput]
Getting dataset basic info...
Getting descriptive statistics for numerical features...
Getting detailed information on categorical variables...
Performing missing values analysis...
Identified numeric columns that should be considered categorical:
['DSEX', 'DETHNIC', 'HYPERTENSION', 'DGRP', 'RSEX', 'RETHNIC', 'GRAFT_NO', 'TX_YR', 'HLA_MM', 'organ_type', 'ALI_0', 'OKI_0', 'REJECTION', 'DGF', 'GCENS', 'COF', 'TX_TYPE', 'organs_dntd', 'ORGANS_TXD', 'PAST_DIABETES', 'PAST_HYPERTENSION']
Performing correlation analysis...
Performing potential outliers identification...
Performing duplicate records analysis...
\end{lstlisting}

\toolOut
\begin{lstlisting}[style=codeoutput]
Dataset Shape: 1200 rows and 39 columns
Column Names and Types:
DONOR_ID               int64
DAGE                   int64
DSEX                   int64
DETHNIC              float64
HYPERTENSION         float64
DGRP                   int64
DRET_CREAT           float64
DCOD                   int64
DBMI                 float64
RECIP_ID               int64
RAGE                   int64
RSEX                   int64
RETHNIC              float64
RBMI                 float64
PRD                    int64
WAIT_TIME            float64
GRAFT_NO               int64
TX_ID                  int64
TX_YR                  int64
HLA_MM               float64
CIT_MINS             float64
CRF_TX                 int64
organ_type             int64
ALI_0                float64
OKI_0                float64
eGFR3                float64
eGFR12               float64
REJECTION            float64
DGF                  float64
GSURV                float64
GCENS                float64
COF                  float64
RCOD                 float64
TX_TYPE                int64
organs_dntd            int64
ORGANS_TXD             int64
PAST_DIABETES        float64
PAST_HYPERTENSION    float64
recip_first_Bw        object

Descriptive Statistics for Numerical Features:
[shortened here for brevity]
            DONOR_ID         DAGE         DSEX     ...   ORGANS_TXD  PAST_DIABETES  PAST_HYPERTENSION
count    1200.000000  1200.000000  1200.000000     ...  1200.000000    1162.000000        1153.000000
mean    64055.581667    44.575833     1.464167     ...     3.371667       1.036145           1.193408
std     13818.714125    16.002531     0.498922     ...     1.168904       0.186730           0.395142
[...]

Identified numeric value columns that should most likely be considered categoricals:
['DSEX', 'DETHNIC', 'HYPERTENSION', 'DGRP', 'RSEX', 'RETHNIC', 'GRAFT_NO', 'TX_YR', 'HLA_MM', 'organ_type', 'ALI_0', 'OKI_0', 'REJECTION', 'DGF', 'GCENS', 'COF', 'TX_TYPE', 'organs_dntd', 'ORGANS_TXD', 'PAST_DIABETES', 'PAST_HYPERTENSION'].
This is done by checking whether the column contains only integers and has a low number of unique values (<20 or <5% of total examples).

Detailed Information on Categorical Variables:
ALI_0 - Unique Values: 2 
Top 5 Values:
ALI_0
1.0    1157
2.0      37

PAST_HYPERTENSION - Unique Values: 2 
Top 5 Values:
PAST_HYPERTENSION
1.0    930
2.0    223

DGF - Unique Values: 3 
Top 5 Values:
DGF
1.0    544
2.0    234
3.0     38

... shortened for brevity ...

RSEX - Unique Values: 2 
Top 5 Values:
RSEX
1    718
2    482

HLA_MM - Unique Values: 0 
Top 5 Values:
Series([], )

DETHNIC - Unique Values: 5 
Top 5 Values:
DETHNIC
1.0    1153
2.0      18
3.0      14
6.0       6
7.0       3

Missing Values Analysis:
DETHNIC                 6
HYPERTENSION           85
DRET_CREAT            129
DBMI                   60
RETHNIC                19
RBMI                  850
HLA_MM               1200
CIT_MINS               16
ALI_0                   6
OKI_0                   6
eGFR3                 237
eGFR12                201
REJECTION              79
DGF                   384
GSURV                   3
GCENS                   3
COF                   758
RCOD                 1043
PAST_DIABETES          38
PAST_HYPERTENSION      47
recip_first_Bw        139

Count of columns with all NaN values: 1
Correlation Analysis:

Most Positively Correlated Features:
     Feature 1   Feature 2  Correlation
0     DONOR_ID       TX_ID     0.998883
1        TX_ID       TX_YR     0.992814
2     DONOR_ID       TX_YR     0.987671
3  organs_dntd  ORGANS_TXD     0.888917
4        eGFR3      eGFR12     0.863228
5     GRAFT_NO      CRF_TX     0.650389
6     DONOR_ID      CRF_TX     0.479641
7        TX_ID      CRF_TX     0.476370
8        TX_YR      CRF_TX     0.468359
9     DONOR_ID    GRAFT_NO     0.432044

Most Negatively Correlated Features:
      Feature 1  Feature 2  Correlation
0      RECIP_ID   GRAFT_NO    -0.684438
1      RECIP_ID     CRF_TX    -0.525426
2         GSURV      GCENS    -0.498340
3      DONOR_ID      GSURV    -0.467702
4         TX_ID      GSURV    -0.467199
5         TX_YR      GSURV    -0.461306
6  HYPERTENSION       DGRP    -0.455477
7          DAGE     eGFR12    -0.450558
8      RECIP_ID  WAIT_TIME    -0.417551
9         GSURV        COF    -0.412299

Outlier Identification for Numerical Features:
DONOR_ID - Outliers Count: 62
[Lower Bound: 2.75e+04, Upper Bound: 9.68e+04]
DAGE - Outliers Count: 0
[Lower Bound: -6.25, Upper Bound: 97.2]
DSEX - Outliers Count: 0
[Lower Bound: -1.75, Upper Bound: 2.75]
... shortened for brevity ...
ORGANS_TXD - Outliers Count: 103
[Lower Bound: 0.25, Upper Bound: 4.75]
PAST_DIABETES - Outliers Count: 80
[Lower Bound: 0, Upper Bound: 0]
PAST_HYPERTENSION - Outliers Count: 270
[Lower Bound: 0, Upper Bound: 0]

Duplicate Records: 0
\end{lstlisting}

\toolReport \\

Here is a correlogram showing the correlation between features: \\

\includegraphics[width=0.8\linewidth]{Log/correlogram.png} \\

A correlogram is a visual tool that shows the relationships between different variables (or features) in a dataset. It presents a grid of color-coded squares, where each square represents the strength and direction of the relationship between two variables. Brighter or darker colors indicate stronger relationships. Positive relationships (where variables increase together) and negative relationships (where one variable increases as the other decreases) are shown with different colors. Here we use reds to denote positive, and blue to denote negative relationships. This makes it easy to see which pairs of variables are related, and how closely they are connected.

\end{toolbox}

\noindent Notice that \textit{CliMB} tools are able to produce a report that may include text and figures, in order to enhance the user's understanding of the results of the tool execution.

\begin{assistantbox}
\assistant The Exploratory Data Analysis (EDA) on your dataset has provided a comprehensive overview, revealing various insights. Here's a summary of the key findings: \\

\begin{enumerate}
    \item Dataset Structure: The dataset consists of 1200 rows and 39 columns after preprocessing. It includes both numerical and categorical variables, providing a rich set of features for analysis.
    \item Descriptive Statistics: Numerical features show a wide range of distributions and scales, indicating the diversity of the data. For instance, variables like \texttt{DONOR\_ID}, \texttt{TX\_ID}, and \texttt{TX\_YR} are highly correlated, suggesting a relationship between donor identification, transaction ID, and the transaction year. Variables like \texttt{eGFR3} and \texttt{eGFR12} (which are of primary interest) also show a strong positive correlation, indicating that early graft function could be predictive of the 12-month graft function.
    \item Categorical Variables: Several categorical variables have been identified, including \texttt{DSEX}, \texttt{DETHNIC}, \texttt{HYPERTENSION}, and \texttt{REJECTION}, among others. These variables show a variety of distributions across their categories, which could be influential in predicting the outcome variable.
    \item Missing Values: The analysis identified missing values in several columns, such as \texttt{DETHNIC}, \texttt{HYPERTENSION}, \texttt{DRET\_CREAT}, and notably, \texttt{HLA\_MM}, which is completely missing. This highlights areas where data imputation or exclusion strategies may be necessary.
    \item Outliers and Duplicates: Outlier detection revealed outliers in many numerical features, which may need to be addressed to prevent skewed analysis. No duplicate records were found, indicating good data integrity.
    \item Correlation Analysis: The correlation analysis highlighted both positive and negative correlations between features. Notably, \texttt{DONOR\_ID}, \texttt{TX\_ID}, and \texttt{TX\_YR} are among the most positively correlated features, while variables like \texttt{GSURV} and \texttt{GCENS} show significant negative correlation, indicating potential areas of interest for further analysis.
    \item Potential Issues for Modeling: The presence of highly correlated features, missing values, and outliers could pose challenges for modeling. Particularly, the identification of numeric columns that should be considered as categorical suggests that encoding strategies may be necessary.
\end{enumerate}

This EDA has provided a foundational understanding of the dataset's structure, content, and potential challenges. It's crucial to consider these insights when moving forward with data preprocessing, feature selection, and modeling to address your research question effectively. \\

Next, I'll proceed with generating descriptive statistics to further understand the dataset's characteristics.
\end{assistantbox}

\begin{toolbox}
\toolExecOut{descriptive\_statistics} \\

\toolLogs
\begin{lstlisting}[style=codeoutput]
Creating the descriptive statistics table...
Saving the summary table to:
[...]/session_2024-08-28_21-18-33/kidney_train_user_cols.csv__descriptive_stats.csv
Identified numeric columns that should be considered categorical:
['DSEX', 'DETHNIC', 'HYPERTENSION', 'DGRP', 'RSEX', 'RETHNIC', 'GRAFT_NO', 'TX_YR', 'HLA_MM', 'organ_type', 'ALI_0', 'OKI_0', 'REJECTION', 'DGF', 'GCENS', 'COF', 'TX_TYPE', 'organs_dntd', 'ORGANS_TXD', 'PAST_DIABETES', 'PAST_HYPERTENSION']
Creating plots for the data...
Normally distributed features:
['RBMI']
Not normally distributed features:
['CIT_MINS', 'CRF_TX', 'DAGE', 'DBMI', 'DCOD', 'DONOR_ID', 'DRET_CREAT', 'GSURV', 'PRD', 'RAGE', 'RCOD', 'RECIP_ID', 'TX_ID', 'WAIT_TIME', 'eGFR12', 'eGFR3']
Plotted a bar plot for: 'ALI_0'
Plotted a bar plot for: 'COF'
Plotted a bar plot for: 'DETHNIC'
... shortened for brevity ...
Plotted a histogram and box plot for: 'WAIT_TIME'
Plotted a histogram and box plot for: 'eGFR12'
Plotted a histogram and box plot for: 'eGFR3'
\end{lstlisting}

\toolOut
\begin{lstlisting}[style=codeoutput]
Variable                  Summary
DONOR_ID             59766 (54447 - 69865)
DAGE                    47.0 (34.0 - 57.0)
DSEX                                      
    1                      643/1200 (53.6)
    2                      557/1200 (46.4)
DETHNIC                                   
    1.0                   1153/1194 (96.6)
    2.0                      18/1194 (1.5)
    3.0                      14/1194 (1.2)
    6.0                       6/1194 (0.5)
    7.0                       3/1194 (0.3)
... shortened for brevity ...
PAST_DIABETES                             
    1.0                   1120/1162 (96.4)
    2.0                      42/1162 (3.6)
PAST_HYPERTENSION                         
    1.0                    930/1153 (80.7)
    2.0                    223/1153 (19.3)
recip_first_Bw                            
    Bw4                    668/1061 (63.0)
    Bw6                    393/1061 (37.0)

The following plots have also been created and saved:
- ALI_0: descr__bar_plot__ALI_0.png
- COF: descr__bar_plot__COF.png
- DETHNIC: descr__bar_plot__DETHNIC.png
... shortened for brevity ...
- WAIT_TIME: descr__hist_box_plot__WAIT_TIME.png
- eGFR12: descr__hist_box_plot__eGFR12.png
- eGFR3: descr__hist_box_plot__eGFR3.png
\end{lstlisting}

\toolReport \\
To view the plots, please select any of the images in the "Working Directory" tab on the right.
\end{toolbox}

\begin{assistantbox}
\assistant The descriptive statistics generated provide a detailed summary of both numerical and categorical variables in your dataset. Here's a concise overview of the findings:

\begin{enumerate}
    \item Numerical Variables: The summary includes median values (or mean where applicable) along with the interquartile range for numerical variables, providing insight into the central tendency and dispersion. For example, \texttt{DAGE} has a median age of 47 years with an interquartile range from 34 to 57 years, indicating the middle 50\% of donor ages.
    \item Categorical Variables: The analysis offers a breakdown of categories within each categorical variable, including counts and percentages. For instance, for \texttt{DSEX} (donor sex), 53.6\% are coded as '1' (possibly male), and 46.4\% as '2' (possibly female).
    \item Missing Data: The summary highlights variables with missing values, which will need to be addressed during data preprocessing. For example, variables like \texttt{HYPERTENSION} and \texttt{DRET\_CREAT} have missing values that could impact the analysis if not handled properly.
    \item Potential Issues: Some variables, such as \texttt{HLA\_MM}, are completely missing, and others like \texttt{RBMI} have a significant percentage of missing data. Additionally, the identification of variables that are numerical but likely represent categorical data (e.g., \texttt{DSEX}, \texttt{organ\_type}) suggests that encoding or transformation might be necessary for proper analysis.
    \item Outliers: The summary identifies outliers in several variables, which may need to be considered during data preprocessing to ensure they do not skew the analysis.
\end{enumerate}

This comprehensive summary provides a solid foundation for understanding the dataset's structure, the distribution of variables, and areas that may require attention during preprocessing, such as missing data handling and outlier management. \\

To further assist in the analysis, here are the five most important figures generated by the descriptive statistics tool, showcasing distributions and relationships within the data: \\

1. Histogram and Box Plot for eGFR12 (graft function at 12 months): \\
\includegraphics[width=1.0\linewidth]{Log/ds1.png}

2. Bar Plot for DSEX (Donor Sex): \\
\includegraphics[width=0.66\linewidth]{Log/ds2.png}

3. Bar Plot for REJECTION (Rejection of Transplant): \\
\includegraphics[width=0.66\linewidth]{Log/ds3.png}

4. Histogram and Box Plot for DAGE (Donor Age): \\
\includegraphics[width=1.0\linewidth]{Log/ds4.png}

5. Bar Plot for HYPERTENSION (Donor Hypertension): \\
\includegraphics[width=0.66\linewidth]{Log/ds5.png}

These figures provide visual insights into key variables of interest, helping to inform further analysis and modeling efforts.

\end{assistantbox}

\begin{assistantbox}
\assistant \cmark~Task completed
\end{assistantbox}

\mydots

\noindent \textbf{Summary of work after this point:} The system then proceeded to work with the user on the remaining stages of the project: data engineering, model building, and model exploitation.

%-------------
\newpage
\subsubsection*{Example 2: Handling of missing values}

\noindent The following example demonstrates how \textit{CliMB} utilizes a multi-step approach to handling missing data, avoiding common missing data pitfalls, and querying user input when necessary using code generation and available tools.

\mygap

\noindent \textbf{Summary of work up to this point:} User data has been loaded, the alignment between the system's capabilities and the user's intended research question has been confirmed, exploratory data analysis and descriptive statistics generation have been completed, and background information about different columns has been discussed with the user.

\noindent At this point, the dataset has 36 columns, 1200 rows, and 5309 (11.3\% of total) missing values.

\mydots

\begin{assistantbox}
\assistant Given the information from the previous steps and the data processing tasks ahead, we'll start by addressing the first subtask, which involves representing any missing data as \texttt{numpy.nan} values. This step ensures that the dataset is correctly prepared for handling missing data in subsequent analyses. \\

From the EDA and descriptive statistics, we observed certain columns with missing values. However, before proceeding to handle these missing values, it's essential to ensure that all missing data, including any non-standard NaN representations, are correctly identified as \texttt{numpy.nan}. \\

Let's generate code to check for non-standard missing values (such as empty strings, placeholders like "NA" or "unknown") and replace them with \texttt{numpy.nan}. This action will standardize the representation of missing data across the dataset. \\

\generatedCode
\begin{lstlisting}
import pandas as pd
import numpy as np

# Load the dataset
data = pd.read_csv("kidney_train_user_cols_corrected_dtypes.csv")

# Replace non-standard NaNs (if any, like 'NA', 'unknown', empty strings) with numpy.nan
# This example shows common placeholders, adjust as necessary based on dataset specifics
non_standard_nans = ['', 'NA', 'unknown']
data.replace(non_standard_nans, np.nan, inplace=True)

# Save the modified dataset
modified_file_path = "kidney_train_user_cols_corrected_dtypes_nan.csv"
data.to_csv(modified_file_path, index=False)

print("Non-standard NaNs (if present) have been replaced with numpy.nan.")
\end{lstlisting}

\end{assistantbox}

\begin{execbox}
\codeExecOut
\codeExecSuccess
\begin{lstlisting}[style=codeoutput]
Non-standard NaNs (if present) have been replaced with numpy.nan.
\end{lstlisting}
\end{execbox}

\noindent In the above step the system first checks for any likely missing value indicators in the dataset, given the analysis so far, and replaces them with \texttt{numpy.nan} to standardize missing value representation. In the subsequent step, the missingness per column is evaluated with the user, and a decision on handling columns with high missingness is made.

\begin{assistantbox}
\assistant Moving on to the next subtask, we will consider dropping columns with high percentages of missing values. To do this, I'll first generate code to calculate and display the percentage of missing values for each column in the dataset. This will help us identify columns that may not contribute valuable information to the analysis due to a high proportion of missing data. \\

Based on the rule of thumb that columns with 80\% or more missing values are candidates for removal, we will review the results and then decide which columns, if any, should be dropped from the dataset. \\

Let's proceed with generating the code to calculate the percentage of missing values per column. \\

\generatedCode
\begin{lstlisting}
import pandas as pd

# Load the dataset
data = pd.read_csv("kidney_train_user_cols_corrected_dtypes_nan.csv")

# Calculate the percentage of missing values for each column
missing_percentage = data.isnull().mean() * 100

# Display the percentage of missing values per column
print("Percentage of missing values per column:")
print(missing_percentage)
\end{lstlisting}

\end{assistantbox}

\begin{execbox}
\codeExecOut
\codeExecSuccess
\begin{lstlisting}[style=codeoutput]
Percentage of missing values per column:
DONOR_ID               0.000000
DAGE                   0.000000
DSEX                   0.000000
DETHNIC                0.500000
HYPERTENSION           7.083333
DGRP                   0.000000
DRET_CREAT            10.750000
DCOD                   0.000000
DBMI                   5.000000
RECIP_ID               0.000000
RAGE                   0.000000
RSEX                   0.000000
RETHNIC                1.583333
RBMI                  70.833333
PRD                    0.000000
WAIT_TIME              0.000000
GRAFT_NO               0.000000
TX_ID                  0.000000
TX_YR                  0.000000
HLA_MM               100.000000
CIT_MINS               1.333333
CRF_TX                 0.000000
organ_type             0.000000
ALI_0                  0.500000
OKI_0                  0.500000
eGFR3                 19.750000
eGFR12                16.750000
REJECTION              6.583333
DGF                   32.000000
GSURV                  0.250000
GCENS                  0.250000
COF                   63.166667
RCOD                  86.916667
TX_TYPE                0.000000
organs_dntd            0.000000
ORGANS_TXD             0.000000
PAST_DIABETES          3.166667
PAST_HYPERTENSION      3.916667
recip_first_Bw        11.583333
dtype: float64
\end{lstlisting}
\end{execbox}

\begin{assistantbox}
\assistant Based on the percentage of missing values calculated for each column, it's evident that most columns have less than 80\% missing data. However, there are exceptions:

\begin{itemize}
    \item HLA\_MM: 100\% missing values.
    \item RBMI: 70.83\% missing values.
    \item COF: 63.17\% missing values.
    \item RCOD: 86.92\% missing values.
\end{itemize}

According to the rule of thumb that any columns with 80\%+ missing values should be considered for removal, HLA\_MM and RCOD exceed this threshold. \\

Would you like to proceed with dropping the columns "HLA\_MM" and "RCOD" due to their high percentage of missing values? Additionally, would you like to set a different threshold for considering the removal of other columns, or keep the remaining columns as they are?

\end{assistantbox}

\begin{userbox}
\user No that's fine. Do remove those two.
\end{userbox}


\begin{assistantbox}
\assistant Given your confirmation, I'll now generate code to drop the columns "HLA\_MM" and "RCOD" from the dataset due to their high percentage of missing values. After removing these columns, the modified dataset will be saved, and we can proceed with the next steps in the data processing pipeline.

\generatedCode
\begin{lstlisting}
import pandas as pd

# Load the dataset
data = pd.read_csv("kidney_train_user_cols_corrected_dtypes_nan.csv")

# Drop the columns with high percentage of missing values
columns_to_drop = ["HLA_MM", "RCOD"]
data.drop(columns=columns_to_drop, inplace=True)

# Save the modified dataset
modified_file_name = "kidney_train_user_cols_corrected_dtypes_nan_dropped.csv"
data.to_csv(modified_file_name, index=False)

print(f"Columns {columns_to_drop} have been dropped. Modified dataset saved as {modified_file_name}.")
\end{lstlisting}
\end{assistantbox}

\begin{execbox}
\codeExecOut
\codeExecSuccess
\begin{lstlisting}[style=codeoutput]
Columns ['HLA_MM', 'RCOD'] have been dropped. Modified dataset saved as kidney_train_user_cols_corrected_dtypes_nan_dropped.csv.
\end{lstlisting}
\end{execbox}

\noindent The system then proceeds to investigating the missingness with respect to rows. Together with the user, a decision is made how to handle rows with missing target variable (drop such rows), and for the rest of the covariates (impute them).

\begin{assistantbox}
\assistant With the columns "HLA\_MM" and "RCOD" successfully removed due to their high percentage of missing values, we can now proceed to the next subtask, which involves considering the dropping of rows with missing values. \\

First, I'll generate code to show:

\begin{itemize}
    \item The per-column percentage of missing values (to revisit and confirm current standings after the column removals),
    \item The percentage of total rows that have any missing values.
\end{itemize}

This information will help us understand the extent of missing data across the dataset and make informed decisions about handling rows with missing values, especially concerning the target variable \texttt{eGFR12}. \\

Let's proceed with generating this code. \\

\generatedCode
\begin{lstlisting}
import pandas as pd

# Load the dataset
data = pd.read_csv("kidney_train_user_cols_corrected_dtypes_nan_dropped.csv")

# Calculate the percentage of missing values for each column
missing_percentage = data.isnull().mean() * 100
print("Percentage of missing values per column:")
print(missing_percentage)

# Calculate the percentage of rows with any missing values
rows_with_missing = (data.isnull().any(axis=1).mean()) * 100
print(f"\nPercentage of total rows with any missing values: {rows_with_missing}%")
\end{lstlisting}
\end{assistantbox}

\begin{execbox}
\codeExecOut
\codeExecSuccess
\begin{lstlisting}[style=codeoutput]
Percentage of missing values per column:
DONOR_ID              0.000000
DAGE                  0.000000
DSEX                  0.000000
DETHNIC               0.500000
HYPERTENSION          7.083333
DGRP                  0.000000
DRET_CREAT           10.750000
DCOD                  0.000000
DBMI                  5.000000
RECIP_ID              0.000000
RAGE                  0.000000
RSEX                  0.000000
RETHNIC               1.583333
RBMI                 70.833333
PRD                   0.000000
WAIT_TIME             0.000000
GRAFT_NO              0.000000
TX_ID                 0.000000
TX_YR                 0.000000
CIT_MINS              1.333333
CRF_TX                0.000000
organ_type            0.000000
ALI_0                 0.500000
OKI_0                 0.500000
eGFR3                19.750000
eGFR12               16.750000
REJECTION             6.583333
DGF                  32.000000
GSURV                 0.250000
GCENS                 0.250000
COF                  63.166667
TX_TYPE               0.000000
organs_dntd           0.000000
ORGANS_TXD            0.000000
PAST_DIABETES         3.166667
PAST_HYPERTENSION     3.916667
recip_first_Bw       11.583333
dtype: float64

Percentage of total rows with any missing values: 97.33333333333334%
\end{lstlisting}
\end{execbox}


\begin{assistantbox}
\assistant Given that a significant portion of the rows (97.33\%) have some missing values, it's crucial to carefully consider how to handle these missing values without losing a substantial amount of data. Specifically, we need to address missing values in the target variable \texttt{eGFR12} and decide on a strategy for handling missing data in other columns. \\

Since imputing the target variable is not recommended, and given the high percentage of rows with missing values:

\begin{enumerate}
    \item For the target variable \texttt{eGFR12}: We should ask if dropping rows with missing \texttt{eGFR12} values is acceptable. This step is crucial as the target variable directly impacts the analysis's outcomes.
    \item For other columns with missing data: We should consider whether to drop rows with any missing data or use an imputation method to fill in these gaps. Given the high percentage of rows affected, imputation might be a preferable strategy to retain as much data as possible.
\end{enumerate}

Are you okay with dropping rows that have missing values in the target variable \texttt{eGFR12}? \\

Additionally, would you prefer to drop rows with missing data in any column or explore imputation methods to handle these missing values, keeping in mind the high percentage of affected rows?
\end{assistantbox}

\begin{userbox}
\user So let's only drop rows where eGFR12 is missing, and keep the rest for later imputation
\end{userbox}

\begin{assistantbox}
\assistant Following your decision, I'll generate code to drop rows where the target variable \texttt{eGFR12} is missing. This step ensures that our analysis on predicting graft function at 12 months will not be compromised by missing target values. The remaining missing values in other columns will be retained for potential imputation later in the process. \\

Let's proceed with the code to drop rows with missing \texttt{eGFR12} values. \\

\generatedCode
\begin{lstlisting}
import pandas as pd

# Load the dataset
data = pd.read_csv("kidney_train_user_cols_corrected_dtypes_nan_dropped.csv")

# Drop rows where 'eGFR12' is missing
data_cleaned = data.dropna(subset=['eGFR12'])

# Save the modified dataset
modified_file_name = "kidney_train_user_cols_corrected_dtypes_nan_dropped.csv"
data_cleaned.to_csv(modified_file_name, index=False)

print(f"Rows with missing 'eGFR12' values have been dropped. Modified dataset saved as {modified_file_name}.")
\end{lstlisting}

\end{assistantbox}

\begin{execbox}
\codeExecOut
\codeExecSuccess
\begin{lstlisting}[style=codeoutput]
Rows with missing 'eGFR12' values have been dropped. Modified dataset saved as kidney_train_user_cols_corrected_dtypes_nan_dropped.csv.
\end{lstlisting}
\end{execbox}

\begin{assistantbox}
\assistant \cmark~Task completed
\end{assistantbox}

\begin{assistantbox}
\assistant \texttt{Planning step}
\end{assistantbox}

\noindent In the final step of missing value handling below, the system confirms the state of missing values in the current version of the dataset, and invokes the HyperImpute imputation tool to complete this step of the workflow.

\begin{assistantbox}
\assistant Before proceeding with imputation, let's first understand the current state of missing values in your dataset after the previous steps. This will involve generating code to calculate and display the percentage of missing values per column and the percentage of total rows that have missing values. This information is crucial for determining the appropriate imputation strategy. \\

After reviewing the missing values, I will explain the HyperImpute tool and its capabilities for imputing missing data. This tool utilizes advanced machine learning algorithms to predict and fill in missing values based on the information available in other columns, potentially preserving the integrity and utility of your dataset for analysis. \\

Let's begin by generating the code to calculate and display the missing values information. \\

\generatedCode
\begin{lstlisting}
import pandas as pd

# Load the dataset
data = pd.read_csv("kidney_train_user_cols_corrected_dtypes_nan_dropped.csv")

# Calculate the percentage of missing values for each column
missing_percentage = data.isnull().mean() * 100

# Calculate the percentage of rows with any missing values
rows_with_missing = (data.isnull().any(axis=1).mean()) * 100

# Display the results
print("Percentage of missing values per column:")
print(missing_percentage)
print(f"\nPercentage of total rows with any missing values: {rows_with_missing}%")
\end{lstlisting}
\end{assistantbox}

\begin{execbox}
\codeExecOut
\codeExecSuccess
\begin{lstlisting}[style=codeoutput]
Percentage of missing values per column:
DONOR_ID              0.000000
DAGE                  0.000000
DSEX                  0.000000
DETHNIC               0.400400
HYPERTENSION          6.606607
DGRP                  0.000000
DRET_CREAT           10.710711
DCOD                  0.000000
DBMI                  4.604605
RECIP_ID              0.000000
RAGE                  0.000000
RSEX                  0.000000
RETHNIC               1.401401
RBMI                 70.970971
PRD                   0.000000
WAIT_TIME             0.000000
GRAFT_NO              0.000000
TX_ID                 0.000000
TX_YR                 0.000000
CIT_MINS              0.900901
CRF_TX                0.000000
organ_type            0.000000
ALI_0                 0.200200
OKI_0                 0.200200
eGFR3                11.711712
eGFR12                0.000000
REJECTION             4.204204
DGF                  31.231231
GSURV                 0.100100
GCENS                 0.100100
COF                  71.071071
TX_TYPE               0.000000
organs_dntd           0.000000
ORGANS_TXD            0.000000
PAST_DIABETES         2.402402
PAST_HYPERTENSION     3.403403
recip_first_Bw       12.112112
dtype: float64

Percentage of total rows with any missing values: 96.7967967967968%
\end{lstlisting}
\end{execbox}

\begin{assistantbox}
\assistant Now that we've identified the current state of missing data in your dataset, let's discuss the next steps for handling these missing values. \\

The HyperImpute tool employs advanced machine learning algorithms to impute missing values in your dataset. It can handle both numerical and categorical data by learning patterns from the available data and using these patterns to predict and fill in missing values. This process can help retain valuable data for analysis, which might otherwise be lost if rows with missing values were simply removed. \\

Before proceeding with the imputation, it's important to note that the HyperImpute tool requires that there are no entirely empty columns in the dataset. We've already addressed columns with a high percentage of missing values, so we should meet this requirement. \\

Are you okay with using the HyperImpute tool to impute the missing values in your dataset, given its capabilities and requirements?
\end{assistantbox}

\begin{userbox}
\user Yes
\end{userbox}

\begin{toolbox}
\toolExecOut{hyperimpute\_imputation} \\

\toolLogs
\begin{lstlisting}[style=codeoutput]
Imputing all columns
Setting up HyperImpute Imputer...
Imputing data...

Missing values before imputation:
DONOR_ID               0
DAGE                   0
DSEX                   0
DETHNIC                4
HYPERTENSION          66
DGRP                   0
DRET_CREAT           107
DCOD                   0
DBMI                  46
RECIP_ID               0
RAGE                   0
RSEX                   0
RETHNIC               14
RBMI                 709
PRD                    0
WAIT_TIME              0
GRAFT_NO               0
TX_ID                  0
TX_YR                  0
CIT_MINS               9
CRF_TX                 0
organ_type             0
ALI_0                  2
OKI_0                  2
eGFR3                117
eGFR12                 0
REJECTION             42
DGF                  312
GSURV                  1
GCENS                  1
COF                  710
TX_TYPE                0
organs_dntd            0
ORGANS_TXD             0
PAST_DIABETES         24
PAST_HYPERTENSION     34
recip_first_Bw       121
dtype: int64
HyperImpute: Iterations completed 1/5
HyperImpute: Iterations completed 2/5
HyperImpute: Iterations completed 3/5
HyperImpute: Iterations completed 4/5
HyperImpute: Iterations completed 5/5

Saving imputation model to:[...]/session_2024-08-22_11-56-14/hyperimpute__kidney_train_user_cols_imputed.pkl

Missing values after imputation:
DONOR_ID             0
DAGE                 0
DSEX                 0
DETHNIC              0
HYPERTENSION         0
DGRP                 0
DRET_CREAT           0
DCOD                 0
DBMI                 0
RECIP_ID             0
RAGE                 0
RSEX                 0
RETHNIC              0
RBMI                 0
PRD                  0
WAIT_TIME            0
GRAFT_NO             0
TX_ID                0
TX_YR                0
CIT_MINS             0
CRF_TX               0
organ_type           0
ALI_0                0
OKI_0                0
eGFR3                0
eGFR12               0
REJECTION            0
DGF                  0
GSURV                0
GCENS                0
COF                  0
TX_TYPE              0
organs_dntd          0
ORGANS_TXD           0
PAST_DIABETES        0
PAST_HYPERTENSION    0
recip_first_Bw       0
dtype: int64

Saving imputed data...
\end{lstlisting}

\toolOut
\begin{lstlisting}[style=codeoutput]
2321 missing values were imputed. The imputed data has been saved to [...]/session_2024-08-22_11-56-14/kidney_train_user_cols_imputed.csv
\end{lstlisting}

\end{toolbox}

\noindent At this point, the dataset has 37 columns (the two 80\%+ missing columns having been removed), 999 rows (the missing target rows having been removed), and no missing values - as one would expect after a successful missing data imputation step.

\mydots

\noindent \textbf{Summary of work after this point:} The system then proceeds to work with the user through the machine learning study, and subsequent post-hoc interpretability including feature importance and subgroup analysis by \texttt{DSEX}.














% \begin{table}[h!]
% \centering

% % Increase row height
% \renewcommand{\arraystretch}{1.15}

% \small

% \begin{tabular}{L{2.6cm}|L{2.8cm}|L{7.8cm}|L{1.5cm}}
% \hline
% \textbf{Project stage} & \textbf{Task name} & \textbf{Subtask name} & \textbf{Subtask selection} \\
% \hline

% \multirow{6}{*}{Alignment check} 
% & \multirow{3}{=}{Getting the environment ready} 
% & Upload data file & mandatory \\
% & & Check hardware & mandatory \\
% & & Check data file can be loaded & mandatory \\
% \cline{2-4}
% & \multirow{3}{=}{Getting information from the user} 
% & High-level information from the user & mandatory \\
% & & Experiment setup and research question from the user & mandatory \\
% & & Assess data suitability and tool support & mandatory \\
% \hline

% \multirow{5}{*}{Data exploration} 
% & \multirow{5}{=}{Exploratory Data Analysis} 
% & Exclude/keep columns & mandatory \\
% & & Perform EDA & mandatory \\
% & & Generate descriptive statistics & mandatory \\
% & & Warn about small sample size if necessary & mandatory \\
% & & Show Kaplan-Meier plot & conditional \\
% \hline

% \multirow{7}{*}{Data engineering} 
% & Data processing - before missing data 
% & Column background information & mandatory \\
% \cline{2-4}
% & \multirow{4}{=}{Data processing - missing data handling} 
% & Represent missing data as NaN & mandatory \\
% & & Consider dropping columns with high missing values & mandatory \\
% & & Consider dropping rows with missing values & mandatory \\
% & & Impute missing values & conditional \\
% \cline{2-4}
% & \multirow{2}{=}{Data processing - after missing data} 
% & Discuss data preprocessing with the user & mandatory \\
% & & Feature selection & mandatory \\
% \hline

% \multirow{7}{*}{Model building} 
% & \multirow{7}{=}{Machine learning study} 
% & Confirm ML problem type & mandatory \\
% & & Check time and event columns & conditional \\
% & & List and confirm features & mandatory \\
% & & Machine learning study - classification & conditional \\
% & & Machine learning study - regression & conditional \\
% & & Machine learning study - survival analysis & conditional \\
% & & Iterate with the user & mandatory \\
% \hline

% \multirow{3}{*}{Model exploitation} 
% & \multirow{3}{=}{Machine learning study} 
% & Feature importance plots & mandatory \\
% & & Insights on classification & conditional \\
% & & Subgroup analysis & mandatory \\
% \hline

% End of Study 
% & Finish up the project 
% & Discuss the project and finish up & mandatory \\
% \hline

% \end{tabular}
% \caption{\textbf{Structured project plan}. This table summarizes all stages, tasks, and subtasks}
% \label{tabplan}
% \end{table}










\begin{table}[h!]
\centering
\small

% Increase row height
\renewcommand{\arraystretch}{1.1}

\begin{tabular}{p{2.3cm}|>{\RaggedRight\arraybackslash}p{2.5cm}|p{7.5cm}|p{1.5cm}}

\hline
\textbf{Project stage} & \textbf{Task name} & \textbf{Subtask name} & \textbf{Subtask selection} \\
\hline

\multirow{6}{=}{Alignment check} 
& \multirow{3}{=}{Getting the environment ready} 
& Upload data file & mandatory \\
& & Check hardware & mandatory \\
& & Check data file can be loaded & mandatory \\
\cline{2-4}
& \multirow{3}{=}{Getting information from the user} 
& High-level information from the user & mandatory \\
& & Experiment setup and research question from the user & mandatory \\
& & Assess data suitability and tool support & mandatory \\
\hline

\multirow{5}{=}{Data exploration} 
& \multirow{5}{=}{Exploratory Data Analysis} 
& Exclude/keep columns & mandatory \\
& & Perform EDA & mandatory \\
& & Generate descriptive statistics & mandatory \\
& & Warn about small sample size if necessary & conditional \\
& & Show Kaplan-Meier plot & mandatory \\
\hline

\multirow{7}{=}{Data engineering} 
& Data processing - before missing 
& Column background information & mandatory \\
\cline{2-4}
& \multirow{4}{=}{Data processing - missing data handling} 
& Represent missing data as NaN & mandatory \\
& & Consider dropping columns with high missing values & mandatory \\
& & Consider dropping rows with missing values & mandatory \\
& & Impute missing values & conditional \\
\cline{2-4}
& \multirow{2}{=}{Data processing - after missing} 
& Discuss data preprocessing with the user & mandatory \\
& & Feature selection & mandatory \\
\hline

\multirow{8}{=}{Model building} 
& \multirow{4}{=}{Machine learning study pre-checks} 
& Confirm ML problem type & mandatory \\
& & Check time and event columns & conditional \\
& & Check for data leakage & mandatory \\
& & Check for irrelevant columns & mandatory \\
\cline{2-4}
& \multirow{3}{=}{Machine learning study} 
& Machine learning study - classification & conditional \\
& & Machine learning study - regression & conditional \\
& & Machine learning study - survival analysis & conditional \\
\cline{2-4}
& Machine learning study iteration 
& Iterate with the user & mandatory \\
\hline

\multirow{3}{=}{Model exploitation} 
& \multirow{3}{=}{Machine learning study exploitation} 
& Feature importance plots & mandatory \\
& & Insights on classification & conditional \\
& & Subgroup analysis & mandatory \\
\hline

End of Study 
& Finish up the project 
& Discuss the project and finish up & mandatory \\
\hline

\end{tabular}

\caption{\textbf{Structured project plan}. This table summarizes all stages, tasks, and subtasks.}
\label{tabplan}
\end{table}
